Construction of Paired Knowledge Graph-Text Datasets Informed by Cyclic Evaluation

Datasets that pair Knowledge Graphs (KG) and text together (KG-T) can be used to train forward and reverse neural models that generate text from KG and vice versa. However models trained on datasets where KG and text pairs are not equivalent can suffer from more hallucination and poorer recall. In this paper, we verify this empirically by generating datasets with different levels of noise and find that noisier datasets do indeed lead to more hallucination. We argue that the ability of forward and reverse models trained on a dataset to cyclically regenerate source KG or text is a proxy for the equivalence between the KG and the text in the dataset. Using cyclic evaluation we find that manually created WebNLG is much better than automatically created TeKGen and T-REx. Guided by these observations, we construct a new, improved dataset called LAGRANGE using heuristics meant to improve equivalence between KG and text and show the impact of each of the heuristics on cyclic evaluation. We also construct two synthetic datasets using large language models (LLMs), and observe that these are conducive to models that perform significantly well on cyclic generation of text, but less so on cyclic generation of KGs, probably because of a lack of a consistent underlying ontology.

==> Sections/abstract.tex <==
\begin{abstract}
% Several datasets such as WebNLG, TekGen, WebGraph, KGPT and T-REx, that match knowledge graphs to natural language sentences have been released recently.
% These datasets can be used to develop neural models that can generate natural language from knoweldge graphs and vice versa. 
% Unfortunately, the manually created datasets are relatively small, with limited ontologies, while the automatically constructed datasets are often plagued with quality issues resulting from spurious alignments and insufficient coverage of the sentences with appropriate graph triples.
% In this paper, we propose that a (KG, text) dataset is of better quality if sentences and graphs that are paired together have almost the same information content in them. We first show that, under this assumption, manually constructed WebNLG is of a much higher quality than automatically constructed datasets, such as TekGen etc. We then propose a multi-step method to automatically create a higher quality dataset using a combination of techniques aimed at improving this equivalence and show how each of these steps improve the quality of the datasets. We also release this dataset, called LAGRANGE.

Recently several datasets have been released that align knowledge graphs (KG) to natural language sentences, such as WebNLG, TeKGen, WebGraph, KGPT, and T-REx. These include both  manually and automatically constructed datasets. This data can be used to train neural models to generate natural language from knowledge graphs and vice versa. These datasets however, suffer from a range of issues such as small dataset size, spurious alignments, and insufficient sentence-graph coverage that can affect the quality trained models. In this paper, we propose that a higher-quality KG-and-text-aligned dataset should have closely matched information content between paired sentences and graphs and propose to use cyclic generation as a means to judge quality. We use this metric to demonstrate the superiority of manually constructed WebNLG over automatically constructed datasets like TekGen. Further, we release a new dataset named LAGRANGE that is created using several heuristics that improve this equivalence.


%-- better coverage during initial alignment of text to knowledge graphs, the use of entailment models and other methods for filtering poor matches, and finally augmentation of the aligned data using a text-to-graph model trained on the data to improve coverage.
%by using a cyclic evaluation -- generating sentences from graphs and using generated sentences to construct the graphs back again, and similarly starting from sentences, generating graphs, which are used to generate the sentences back again. 
\end{abstract}

==> Sections/ack.tex <==
% \section*{Acknowledgements}

==> Sections/intro.tex <==
\section{Introduction}\label{sec:intro}
%The Natural Language Processing community has witnessed an explosion in new tools for language modeling with the introduction of transformers. 
%However, these models encode language within the weights of the parameters of the model, which makes it hard to assess the source of knowledge that they encode.
Knowledge graphs (KGs) are widely used in applications like question answering and recommendation systems, offering a structured representation of information through triples. Each triple expresses a relationship (edge) between a subject entity and an object entity (nodes). 
In addition to developing the tools needed to create KGs, to maintain the provenance of encoded information, and methods to update KGs in near real time, the KG community has also developed automated means to assess triple quality using probabilistic approaches. 
This makes KGs an interesting complement to large language models (LLM). KGs can provide formal guarantees on the quality and provenance of information stored in them, but do not provide an obvious way to interact with natural language. 
Recently there has been an acceleration in attempts to intersect the modalities of natural language and KGs using neural approaches that can be used to generate text conditioned on KG triples or generate / perform retrieval of KG triples conditioned on text. Such models can enable capabilities such as reasoning on KGs. However, these models require supervised data where each example is a pair of a text and associated knowledge sub-graph.
Several efforts, such as TekGen~\citep{tekgen}, KGPT~\citep{kgpt}, TREx~\cite{trex}, and others, have aimed at automatically aligning knowledge graph elements from Wikidata with relevant sentences in Wikipedia. In addition, datasets such as WebNLG~\cite{webnlg} have been constructed manually. Unfortunately, manually created datasets like WebNLG, despite their high quality, are relatively small in comparison to the datasets commonly employed for training NLP algorithms.
The automatically constructed datasets on the other hand, are often plagued with quality issues resulting from poor alignments, and insufficient coverage of the sentences with appropriate sub-graph triples.


In this paper, we argue that a dataset is better if the sentences and the KGs paired with them have the same information content. Models trained on data of better alignment should exhibit less hallucination -- whether generating text from KG or vice versa. The quality of cyclic generation of KG from text, or of text from KG using models trained on a dataset would thus allow us to measure the quality of the dataset itself.
An additional benefit of cyclic evaluations is that it allows us to compare across datasets using different ontologies; this is harder to do when only comparing uni-directional models that generate graph from text or vice versa, because of the peculiarities of the KG ontology or of the sentence styles themselves. We use this method to compare several different available datasets. In light of the success of LLMs in handling KGs, we also construct synthetic (KG, text datasets) from two large language models and assess the utility of these synthetic datasets for our generative tasks.


Finally, we apply our lessons learned to create and release a \textbf{la}rge-scale \textbf{gra}ph-text alig\textbf{n}ed dataset for graph-text cross-modal \textbf{ge}neration (\textbf{LAGRANGE}) that has better equivalence between sentences and KGs compared to the previous datasets. Through extensive experiments, we show how the different heuristics we used to create the dataset have led to the improved quality.



% In this paper, we show how one can assess the quality of the aligned datasets, using the assumption that a dataset is better if the sentences paired with the graphs have almost the same information content in them. 
% This equivalence can be assessed by using two different cyclic evaluations. The first cyclic evaluation (GTG) starts with a knowledge graph, and generates text from it, which in turn is used to reconstruct the knowledge graph back again. 
% The second cyclic evaluation (TGT) starts with text and generates graphs, which are in turn used to generate the sentences back again.
% The equivalence between the source (text or graph) and the corresponding cyclically generated output (text or graph) represents the quality of the datasets, because the generations are performed using two separate models trained on the same data -- one that is trained to generate text from knowledge graphs and another that is trained in reverse, generating knowledge graphs from text. Our assumption is that datasets where text, paired graphs are better matched would produce models that exhibit less hallucination of facts in both directions and resulting in better cyclic results. An additional benefit of cyclic evaluations is that it allows us to compare across datasets using different ontologies, as this is harder to do when only comparing uni-directional models that generate graph from text or vice versa.
% Using this assumption we show that manual datasets such as WebNLG are of much higher quality, while, automatically constructed datasets, though much larger, are much poorer in quality, and training models on them results in much more hallucination.
% We then propose a multi-step method to create a higher quality dataset using a combination of techniques -- better coverage during initial alignment of text to knowledge graphs, the use of entailment models and other methods for filtering poor matches, and finally augmentation of the aligned data using a text-to-graph model trained on the data to improve coverage.
% We show how each of these steps improve the quality of the datasets and release the dataset, which we call LAGRANGE.

%However successful neural models require large datasets and the existing datasets fall short of this goal in various ways.
%For example KGText and TekGen are obtained by aligning first sections of Wikipedia to corresponding entries in Wikidata\citep{wikidata} which is a publicly available Knowledge graph whose entities are closely tied to Wikipedia. 
%As a result the number of triples in the datasets is much smaller than what is available in Wikidata.
%In this paper we present a semi-supervised approach that helps us avoid this limitation. 
%The methods works by creating an initial low precision but high recall alignment of Wikidata triples to Wikipedia using manually defined heuristics.
%Subsequently we use multiple rounds of refinement of this dataset by selecting a high precision subset using an entailment model, which is retrained on progressively larger data, and used to generate the next round of dataset from the low quality super-set. 
%This helps us create a much larger dataset which we call \textbf{\textit{LAGRANGE}} 
%We show the benefits of having a larger dataset by training KG to Text, and KG retrieval models on different existing dataset and assessing the resulting models in two different ways -- zero shot evaluation on an existing dataset called WebNLG, and evalution on a held out test set that was manually labelled by a cloud annotation service. On these evaluations models trained on our data consistently outperform the same models trained on prior data.

==> Sections/lagrange.tex <==
%\section{Construction of Lagrange}\label{sec:improve}

%In this section, we describe the steps used to create Lagrange, with the goal of improving the alignment between KG and text pairs.

\subsubsection{Predicate Entailment}\label{subsec:tf}

As we mentioned in Section \ref{sec:rawdata}, the raw data collection step is mainly focused on having a large recall and hence, we do not perform any predicate matching between the sentence and triples, which results in a certain amount of mismatched triples. To address this issue, we remove the misaligned triples by leveraging a semantic entailment model. In particular, we use a RoBERTa-large \cite{} model fine-tuned on natural language inference (NLI) datasets, including SNLI \cite{snli:emnlp2015}, ANLI \cite{nie2019adversarial} and MNLI \cite{N18-1101}. As depicted in Figure \ref{fig:entail}, the entailment model takes a sentence and a triple as input pairs and computes an entailment score to predict whether the sentence entails the facts described by the triple. We have observed that the prediction accuracy can be influenced by the absence of a subject in the sentence, such as when a pronoun is used as the subject. To tackle this issue, we employ a solution where we prepend the Wikipedia page title to the sentence during the inference process.

\begin{figure}[t]
\centering
\includegraphics[width=0.49\textwidth]{figs/pp.pdf}
\caption{Using the entailment model to filter the sentence-triple pairs.}
\label{fig:entail}
\end{figure}

% Since the entailment model is trained on natural language but the triple in our dataset is structured data, we hope to understand how well it can predict the entailment relation on our data. To measure the accuracy, we launched an annotation effort and manually labeled 10K pairs of sentence and triple from our raw dataset. 


\subsubsection{Second-Hop Neighbors}\label{subsec:sh}

Previous works were mainly focused on extracting first-hop neighbors of subjects in a sentence. However, a significant number of sentences contains additional information about these first-hop neighbors. In this work and as we described in Section \ref{sec:rawdata}, we extend our scope and consider second-hop neighbors as well. More concretely, we consider matching triples from the Wikidata graph of first-hop neighbors of the subject. See Figure \ref{fig:wiki_triples} for examples. We will show in experimental results how including triples from Wikidata graph of first-hop neighbors and considering second-hop neighbors enhance the overall quality of our dataset.


\subsubsection{Sentence Length}\label{subsec:slt}

The Wikipedia corpus contains a substantial number of lengthy sentences. In the case of many of these sentences, we are only able to find a relatively limited number of matching triples. This limitation arises because certain information in sentences cannot be represented within the WikiData ontology. To analyze the statistics, we calculate the length of sentences (measured in terms of the number of words) and plot the average, median, 30\textsuperscript{th} percentile, and 90\textsuperscript{th} percentile against the number of aligned triples. As depicted in Figure \ref{fig:nw_vs_nt}, We observe a roughly linear relationship between the number of aligned triples and the number of words.

To address the misalignment caused by this \textit{unrepresentability} issue, we apply a threshold to the sentence length based on the number of triples. Given that the majority of examples in our dataset consist of a single triple, we impose a more stringent limit on their sentence length. For examples with more than one triple, we restrict the sentence length to the 90\textsuperscript{th} percentile. However, for single-triple examples, we set the length threshold at the 30\textsuperscript{th} percentile.

\begin{figure}[t]
\centering
\hspace*{-0.3cm}
\includegraphics[width=0.4\textwidth]{figs/nw_vs_nt.png}
\caption{The relationship between the number of triples and the number of words in the sentence.}
\label{fig:nw_vs_nt}
\end{figure}

\subsubsection{Triple Augmentation}\label{subsec:ta}

Misalignment can also occur due to missing triples in the dataset. These missing triples can result from either being overlooked during our construction process or not being available on Wikidata. We mitigate this issue by generating the missing triples from the trained T2G models. Since the T2G model is trained on a substantial amount of data, it is capable of  completing missing triples. We apply the T2G model to the training data, collecting the generated \textit{new} triples as an augmentation to the original training set.

% Table \ref{tab:data-features} summarizes these improvement steps and compare our dataset with previous works in terms of them.

==> Sections/legacy/construction.tex <==
\subsection{Raw dataset collection}\label{subsec:rawdata}

In this section, we describe the methodology we used to create our dataset which consists of pairs of aligned graph triples from Wikidata and sentence from Wikipedia. We begin by describing how we have paired Wikipedia sentences with Wikidata triples. Then, we describe the post-processing step we have used to filter out noisy matches. 

\subsection{Triple-Sentence Alignment}\label{subsec:align}

Wikipedia and Wikidata pages are associated with each other through a unique $\qidn$. For each $\qidn$ $\mathtt{q}$, we consider the set of all sentences $\sqid$ from its Wikipedia page. We also consider the set of all triples from the corresponding Wikidata page as $\tqid=\{(s, p, o)\}$ where $s$ denotes the subject or $\mathtt{q}$ title, $p$ denotes the predicate that could be either simple or compound as we will describe later, and $o$ denotes the object. For each sentence in $\sqid$, our goal is to match as many triples as possible from $\tqid$ and neighboring Wikidata graphs to it. Before describing the matching process, we would like to provide more details on how $\tqid$ is built.

For each $\qidn$ $\mathtt{q}$, the subject $s$ in each triple $(s, p, o) \in \tqid$ is always the title of $\mathtt{q}$ (e.g. \textit{Barack Obama} for $\textrm{Q}_{76}$). The object $o$ on the other hand, could be 
\begin{itemize}
\item the title or alias of another $\qidn$. As an example, \textit{Michelle Obama} that is the title of $\textrm{Q}_{13133}$ as in \texttt{(Barack Obama, Spouse, Michelle Obama)}.
\item strings that are not associated to any $\qidn$.  As an example, \textit{Barry} as in \texttt{(Barack Obama, Nickname, Barry)}.
\item literal values such as dates or quantities and their possible aliases. As an example, we have \texttt{(Barack Obama, date of birth, +1961-08-04T00:00:00Z)} on Wikidata. However, on a Wikipedia sentence, this date could be expressed as \texttt{August 4, 1961} or \texttt{Aug 4, 1961}. Hence, we consider different aliases of a literal in order to match more triples.
\end{itemize}
Finally, the predicate $p$ could either be simple as in \texttt{(Barack Obama, Occupation, Lawyer)} or compound as in \texttt{(Barack Obama, Occupation Lawyer Start Time , 1991)}. In other words, if an object of a triple has a qualifier (i.e., an additional predicate and object) itself, we concatenate them using the format of \texttt{predicate1 object1 predicate2} and form a new triple \texttt{(subject, predicate1 object1 predicate2, object2)} in addition to the original triple \texttt{(subject, predicate1, object1)}.



For each sentence \texttt{s} in $\sqid$, we define $\mathcal{M'}_{\mathtt{s},\mathtt{q}}$ as the set of all triples $(s, p, o) \in \tqid$ where $o$ has appeared in the sentence \texttt{s}. In other words, $\mathcal{M'}_{\mathtt{s},\mathtt{q}}$ denotes the set of triples matched to \texttt{s} in which objects are first-hop neighbors of $\mathtt{q}$ in Wikidata graph. As an example, if the sentence \texttt{s} is [\textit{Barack Obama is an American politician who served as the 44th president of the United States from 2009 to 2017.}], then $\texttt{(Barack Obama, Occupation, Politician)} \in \mathcal{M'}_{\mathtt{s},\mathrm{Q_{76}}}$ since the word \texttt{politician} has appeared in the sentence \texttt{s} and the entity \texttt{Politician} (i.e., $\mathrm{Q_{82955}}$) is a first-hop neighbor of \texttt{Barack Obama} (i.e., $\mathrm{Q_{76}}$) on Wikidata. It is noteworthy to mention that at this stage we do not put any constraint on the predicate of matched triples. We will later explain how our post-processing helps us to match predicates as well.


Having constructed the $\mathcal{M'}_{\mathtt{s},\mathtt{q}}$, let $\mathcal{Q}$ denote the set of all $\qidn$s in Wikidata and define $Q_{\mathcal{M'}_{\mathtt{s},\mathtt{q}}}= \{o|(s,p,o)\in {\mathcal{M'}_{\mathtt{s},\mathtt{q}}} \land \exists q'\in \mathcal{Q}: o \equiv q' \}$. In other words, for each sentence \texttt{s} in $\sqid$, $Q_{\mathcal{M'}_{\mathtt{s},\mathtt{q}}}$ denotes the set of all $\qidn$s that have appeared in $\texttt{s}$ in the original or an alias format and are first-hop neighbors of $\mathtt{q}$ in Wikidata. In the aforementioned example where the matched triple \texttt{(Barack Obama, Occupation, Politician)} is in $\mathcal{M'}_{\mathtt{s},\mathrm{Q_{76}}}$, the $\qidn$ corresponding to \texttt{Politician} (i.e., $\texttt{Q}_{82955}$) is also in $Q_{\mathcal{M'}_{\mathtt{s},\mathrm{Q_{76}}}}$. 


\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{figs/wiki_example.pdf}
\caption{Sample sentences and their corresponding subgraphs from Barack Obama's Wikipedia article and Wikidata. Words that are annotated in green and red are first-hop and second-hop neighbors of Barack Obama on Wikidata, respectively.}
\label{fig:wiki_graph}
\end{figure}
\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{figs/wiki_example_2.pdf}
\caption{Example sentences from Barack Obama's Wikipedia article and matched triples to them. Note that our approach goes beyond first-hop neighbors by considering the second-hop neighbors.}
\label{fig:wiki_triples}
\end{figure}



In addition to $\mathcal{M'}_{\mathtt{s},\mathtt{q}}$, we define $\mathcal{M''}_{\mathtt{s},\mathtt{q}}$ as the set of all triples $(s', p', o')$ where $s'\in Q_{\mathcal{M'}_{\mathtt{s},\mathtt{q}}}$ (i.e., subject $s'$ is a $\mathrm{Q_{id}}$ and a first-hop neighbor of $\mathtt{q}$) and $o'$ has appeared in the sentence $\mathtt{s}$. As an example, consider the following sentence $\mathtt{s}$ from Barack Obama's Wikipedia article: [\textit{His mother, Ann Dunham (1942–1995), was born in Wichita, Kansas; she was mostly of English descent.}]. Based on Barack Obama's Wikidata graph, we have $\texttt{(Barack Obama, Mother, Ann Dunham)} \in \mathcal{M'}_{\mathtt{s},\mathrm{Q_{76}}}$ and hence, $\mathrm{Q_{766106}}(\mathrm{Ann~Dunham}) \in Q_{\mathcal{M'}_{\mathtt{s},\mathrm{Q_{76}}}}$. Since \texttt{Ann Dunham} is the first-hop neighbor of \texttt{Barack Obama} and \texttt{Wichita}, \texttt{1942}, \texttt{1995} are the first-hop neighbors of \texttt{Ann Dunham}, then \texttt{(Ann Dunham, Place of Birth, Wichita)}, \texttt{(Ann Dunham, Date of Birth, 1942)}, \texttt{(Ann Dunham, Date of Death, 1995)} are all in $\mathcal{M''}_{\mathtt{s},\mathrm{Q_{76}}}$. Figure \ref{fig:wiki_graph} shows the example sentences from Wikipedia and their corresponding subgraphs from Wikidata. In addition, Figure \ref{fig:wiki_triples} shows the matched triples to each sentence based on the Wikidata subgraphs in Figure \ref{fig:wiki_graph}. As seen in Figure \ref{fig:wiki_triples}, considering second-hop neighbors can significantly increase the number of matched triples and give us a richer dataset for training graph-to-text generative models.

\begin{table}[]
\begin{tabular}{|c||c|c|}
\hline
\textbf{Dataset}                                                      & \multicolumn{1}{l|}{\textbf{\#Sentences}} & \multicolumn{1}{l|}{\textbf{\#Triples}} \\ \hline\hline
KGPT                                                          & 7,000,000                        & 16,000,000                     \\ \hline
TEKGEN                                                        & 7,978,814                        & 16,090,457                     \\ \hline
GenWiki                                                       & 1,336,766                        & 2,607,997                      \\ \hline
\begin{tabular}[c]{@{}c@{}}LAGRANGE\\ pre-filter\end{tabular} & 37,568,527                      & 104,424,740                     \\ \hline
\end{tabular}
\caption{Statistics of our initial dataset and its comparison with other published datasets.}
\label{tab:init}
\end{table}

Once we have both $\mathcal{M'}_{\mathtt{s},\mathtt{q}}$ and $\mathcal{M''}_{\mathtt{s},\mathtt{q}}$, then we build $\mathcal{M}_{\mathtt{s},\mathtt{q}}= \mathcal{M'}_{\mathtt{s},\mathtt{q}} \cup \mathcal{M''}_{\mathtt{s},\mathtt{q}}$ to denote the set of all matched triples from $\mathcal{T}_\mathtt{q}$ to $\mathtt{s}$. As we mentioned before, at this stage we do not put any constraint on matching the predicates and we just care about matching the subject and object of candidate triples with a given sentence. In the next section we describe how our post-processing step filters out triples with non-matching predicates. Table \ref{tab:init} shows the statistics of our initial dataset and its comparison with TEKGEN \citep{tekgen}, KGPT \citep{kgpt}, GenWiki \citep{jin2020genwiki}. Finally, it is noteworthy to mention that 30 million triples in our initial dataset our based on second-hop neighbors of entities. Although our post-processing step filters out a number of these triples, we would like to emphasize on how going beyond first-hop neighbors can give us a dataset with higher quality, unlike other datasets that we have mentioned them in Table \ref{tab:datasets}.


==> Sections/legacy/method.tex <==
\section{Methods}\label{sec:method}

In this section, we describe the methodology we used to create our dataset which consists of pairs of aligned graph triples from Wikidata and sentence from Wikipedia. We begin by describing how we have paired Wikipedia sentences with Wikidata triples. Then, we describe the post-processing step we have used to filter out noisy matches. 

\input{Sections/construction.tex}

\input{Sections/pp.tex}

==> Sections/legacy/pp.tex <==
\subsection{Post-processing}\label{subsec:pp}

In order to improve the quality of matching, we add a post-processing step to remove the misaligned triples to the sentences. As is shown in Figure \ref{fig:entail}, we leverage a pre-trained RoBERTa-large model for text classification, which is further fine-tuned on natural language inference (NLI) datasets, including SNLI, ANLI and MNLI. The post-processing model takes a pair of sentence and triple as inputs and computes a probability as an entailment score to indicate whether the facts described by the triple is entailed by the given sentence. To address the cases where the sentence do not include the subject in the triple but a pronoun or a possessive adjective instead, we prepend the Wikipedia page title to the sentence and connect with a ". ".

\begin{figure}[h]
\centering
\includegraphics[width=0.49\textwidth]{figs/pp.pdf}
\caption{Using the entailment model to filter the sentence-triple pairs.}
\label{fig:entail}
\end{figure}

Since the entailment model is trained on natural language but the triple in our dataset is structured data, we hope to understand how well it can predict the entailment relation on our data. To measure the accuracy, we launched an annotation effort and manually labeled 10K pairs of sentence and triple from our raw dataset. 

Although the entailment model does a great job in filtering out the negative pairs, it misclassifies a significant portion of positive pairs as negative. There is still a large room to improve the accuracy of this model. Considering that large-scale annotated data for model training is not available, we leverage self-supervised learning to further improve the post-processing model. More specifically, we adopt an iterative pseudo-labeling~\cite{lee2013pseudo} approach to fine-tune the entailment model.

\begin{figure*}[h]
\centering
\includegraphics[width=\textwidth]{figs/pseudo_labeling.pdf}
\caption{The iterative entailment fine-tuning based on pseudo labeling.}
\label{fig:iterative}
\end{figure*}


Starting with the raw dataset created in Section \ref{subsec:align} and the baseline entailment model, we score the examples using the model and fine-tune the model with selected examples. This process is repeated in iterations. As is shown in Figure \ref{fig:iterative}, we break each iteration into 4 step:

\begin{enumerate}
  \item Since the entire dataset is too large, we subsample the raw dataset as fine-tuning data for each iteration. Each example is the form of a pair of one sentence and one triple matched to the sentence. For each iteration, we subsample different set of examples in the raw data pool.
  \item We compute the probability of entailment for the triple to the sentence, using the entailment model. This probability of entailment is consider as a score of alignment.
  \item To construct a fine-tuning, we select the pairs with high scores as positive examples and, similarly, the low-score pairs as negative examples. 
  \item With the constructed dataset, we fine-tune the classification head of the baseline, with a batch size of 2048. The fine-tuned model will be used in Step 2 of the next iteration.
\end{enumerate}

We repeat the steps in iterations until the metrics on the human annotated datasets stops improving. However, there are a few issues need to be addressed in order to make a good fine-tuning data. We cover them in more details in Section \ref{subsec:predicates} and \ref{subsec:negsample}.

\subsubsection{Predicate distribution}\label{subsec:predicates}
Given the way how we align the sentences and triples, certain predicate types are more likely to be positive and some others are more often to be negative. For example, triples with predicates \texttt{instance of} or \texttt{occupation} are more often too be positive since if you could match a person's occupation in text, the sentence most likely entails the fast. In contrast, for triples with predicates such as \texttt{place of death}, the places we matched in the sentences are usually not the place of death thus the \texttt{place of death} triples most likely to be negative. 

This nature creates a unbalanced dataset in two ways: 1. for some predicate, the samples can be significantly biased towards the positive (or negative) class; 2. the number of total positive samples is much larger than the number of negative samples. Training on this dataset might lead to a model that: 1. biased to predict more positive labels and 2. learns to make prediction based solely on the predicate (for example, predicting all \texttt{occupation} triples as positive since 90\% of the \texttt{occupation} triples are positive). 

To balance the number of samples, at each iteration, we set a limit of 10K per predicate per class: sampling at most 10K positives and 10K negatives for each predicate. To avoid sampling biased over documents, the subsampled raw data is fully shuffled before the selection.  


\subsubsection{Negative sampling}\label{subsec:negsample}

In order to address the issue of samples biased to the positive class, we include negative sampling when constructing the fine-tuning dataset. As triple in raw data are selected by matching the subject and object, the main challenge is to determine whether the predicate in a triple is entailed by the sentence. Thus, given a positive triple, we replace the predicate by another different one to construct a negative (sentence, triple) pair. 

For negative examples, we replace a predicate with another random predicate to form an "easy" negative example. These "easy" negative examples might be too different from the positive predicate and the paired sentence, so that it could be trivial for the entailment model to differentiate. In this case, we also draw "hard" negative examples from a graph embedding (GE) model. A GE model is trained on Wikidata KG to embed the predicates, in which way we can query the most similar predicates to a given predicate. When constructing a hard negative examples, we use the similar predicates as "hard" negative predicate.

% \begin{figure}[h]
%      \centering
%      \begin{subfigure}
%          \centering
%          \hspace*{-0.9cm}
%          \includegraphics[width=0.6\textwidth]{figs/violin_baseline.pdf}
%          \caption*{Baseline model}
%          \label{fig:entail_score_before}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}
%          \centering
%          \hspace*{-0.9cm}
%          \includegraphics[width=0.6\textwidth]{figs/violin_iterative.pdf}
%          \caption*{Fine-tuned model}
%          \label{fig:entail_score_after}
%      \end{subfigure}
%         \caption{Entailment score distribution before and after fine-tuning.}
%         \label{fig:entail_score}
% \end{figure}


==> Sections/raw_data.tex <==
\section{Datasets}\label{sec:rawdata}

In this section, we describe the methodology used to create Lagrange and the synthetic datasets.

\subsection{Lagrange}
Lagrange consists of pairs of aligned KG triples from Wikidata and sentence from Wikipedia. We begin by describing how we have paired Wikipedia sentences with Wikidata triples. Then, we describe the post-processing step used to filter out noisy matches. 

\subsubsection{Triple-Sentence Alignment}\label{subsec:align}

Wikipedia and Wikidata pages are associated with each other through a unique $\qidn$. For each $\qidn$ $\mathtt{q}$, we consider the set of all sentences $\sqid$ from its Wikipedia page. We also consider the set of all triples from the corresponding Wikidata page as $\tqid=\{(s, p, o)\}$ where $s$ denotes the subject or $\mathtt{q}$ title, $p$ denotes the predicate that could be either simple or compound as we will describe later, and $o$ denotes the object. For each sentence in $\sqid$, our goal is to match as many triples as possible from $\tqid$ and neighboring Wikidata graphs to it. Before describing the matching process, we would like to provide more details on how $\tqid$ is built.

For each $\qidn$ $\mathtt{q}$, the subject $s$ in each triple $(s, p, o) \in \tqid$ is always the title of $\mathtt{q}$ (e.g. \textit{Barack Obama} for $\textrm{Q}_{76}$). The object $o$ on the other hand, could be 
\begin{itemize}
\item the title or an alias of another $\qidn$. As an example, \textit{Michelle Obama} that is the title of $\textrm{Q}_{13133}$ as in \texttt{(Barack Obama, Spouse, Michelle Obama)}.
\item strings that are not associated to any $\qidn$.  As an example, \textit{Barry} as in \texttt{(Barack Obama, Nickname, Barry)}.
\item literal values such as dates or quantities and their possible aliases. As an example, we have \texttt{(Barack Obama, date of birth, +1961-08-04T00:00:00Z)} on Wikidata. However, on a Wikipedia sentence, this date could be expressed as \texttt{August 4, 1961} or \texttt{Aug 4, 1961}. Hence, we consider different aliases of a literal in order to match more triples.
\end{itemize}
Finally, the predicate $p$ could either be simple as in \texttt{(Barack Obama, Occupation, Lawyer)} or compound as in \texttt{(Barack Obama, Occupation Lawyer Start Time , 1991)}. In other words, if an object of a triple has a qualifier (i.e., an additional predicate and object) itself, we concatenate them using the format of \texttt{predicate1 object1 predicate2} and form a new triple \texttt{(subject, predicate1 object1 predicate2, object2)} in addition to the original triple \texttt{(subject, predicate1, object1)}.



For each sentence \texttt{s} in $\sqid$, we define $\mathcal{M'}_{\mathtt{s},\mathtt{q}}$ as the set of all triples $(s, p, o) \in \tqid$ where $o$ has appeared in the sentence \texttt{s}. In other words, $\mathcal{M'}_{\mathtt{s},\mathtt{q}}$ denotes the set of triples matched to \texttt{s} in which objects are first-hop neighbors of $\mathtt{q}$ in Wikidata graph. As an example, if the sentence \texttt{s} is [\textit{Barack Obama is an American politician who served as the 44th president of the United States from 2009 to 2017.}], then $\texttt{(Barack Obama, Occupation, Politician)} \in \mathcal{M'}_{\mathtt{s},\mathrm{Q_{76}}}$ since the word \texttt{politician} has appeared in the sentence \texttt{s} and the entity \texttt{Politician} (i.e., $\mathrm{Q_{82955}}$) is a first-hop neighbor of \texttt{Barack Obama} (i.e., $\mathrm{Q_{76}}$) on Wikidata. It is noteworthy to mention that at this stage we do not put any constraint on the predicate of matched triples. We will later explain how our post-processing helps us to match predicates as well.


Having constructed the $\mathcal{M'}_{\mathtt{s},\mathtt{q}}$, let $\mathcal{Q}$ denote the set of all $\qidn$s in Wikidata and define $Q_{\mathcal{M'}_{\mathtt{s},\mathtt{q}}}= \{o|(s,p,o)\in {\mathcal{M'}_{\mathtt{s},\mathtt{q}}} \land \exists q'\in \mathcal{Q}: o \equiv q' \}$. In other words, for each sentence \texttt{s} in $\sqid$, $Q_{\mathcal{M'}_{\mathtt{s},\mathtt{q}}}$ denotes the set of all $\qidn$s that have appeared in $\texttt{s}$ in the original or an alias format and are first-hop neighbors of $\mathtt{q}$ in Wikidata. In the aforementioned example where the matched triple \texttt{(Barack Obama, Occupation, Politician)} is in $\mathcal{M'}_{\mathtt{s},\mathrm{Q_{76}}}$, the $\qidn$ corresponding to \texttt{Politician} (i.e., $\texttt{Q}_{82955}$) is also in $Q_{\mathcal{M'}_{\mathtt{s},\mathrm{Q_{76}}}}$. 


\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{figs/wiki_example.pdf}
\caption{Sample sentences and their corresponding subgraphs from Barack Obama's Wikipedia article and Wikidata. Words that are annotated in green and red are first-hop and second-hop neighbors of Barack Obama on Wikidata, respectively.}
\label{fig:wiki_graph}
\end{figure}
\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{figs/wiki_example_2.pdf}
\caption{Example sentences from Barack Obama's Wikipedia article and matched triples to them. Note that our approach goes beyond first-hop neighbors by considering the second-hop neighbors.}
\label{fig:wiki_triples}
\end{figure}



In addition to $\mathcal{M'}_{\mathtt{s},\mathtt{q}}$, we define $\mathcal{M''}_{\mathtt{s},\mathtt{q}}$ as the set of all triples $(s', p', o')$ where $s'\in Q_{\mathcal{M'}_{\mathtt{s},\mathtt{q}}}$ (i.e., subject $s'$ is a $\mathrm{Q_{id}}$ and a first-hop neighbor of $\mathtt{q}$) and $o'$ has appeared in the sentence $\mathtt{s}$. As an example, consider the following sentence $\mathtt{s}$ from Barack Obama's Wikipedia article: [\textit{His mother, Ann Dunham (1942–1995), was born in Wichita, Kansas; she was mostly of English descent.}]. Based on Barack Obama's Wikidata graph, we have $\texttt{(Barack Obama, Mother, Ann Dunham)} \in \mathcal{M'}_{\mathtt{s},\mathrm{Q_{76}}}$ and hence, $\mathrm{Q_{766106}}(\mathrm{Ann~Dunham}) \in Q_{\mathcal{M'}_{\mathtt{s},\mathrm{Q_{76}}}}$. Since \texttt{Ann Dunham} is the first-hop neighbor of \texttt{Barack Obama} and \texttt{Wichita}, \texttt{1942}, \texttt{1995} are the first-hop neighbors of \texttt{Ann Dunham}, then \texttt{(Ann Dunham, Place of Birth, Wichita)}, \texttt{(Ann Dunham, Date of Birth, 1942)}, \texttt{(Ann Dunham, Date of Death, 1995)} are all in $\mathcal{M''}_{\mathtt{s},\mathrm{Q_{76}}}$. Figure \ref{fig:wiki_graph} shows the example sentences from Wikipedia and their corresponding subgraphs from Wikidata. In addition, Figure \ref{fig:wiki_triples} shows the matched triples to each sentence based on the Wikidata subgraphs in Figure \ref{fig:wiki_graph}. As seen in Figure \ref{fig:wiki_triples}, considering second-hop neighbors can significantly increase the number of matched triples and give us a richer dataset for training graph-to-text generative models.

% \begin{table}[]
% \begin{tabular}{|c||c|c|}
% \hline
% \textbf{Dataset}                                                      & \multicolumn{1}{l|}{\textbf{\#Sentences}} & \multicolumn{1}{l|}{\textbf{\#Triples}} \\ \hline\hline
% KGPT                                                          & 7,000,000                        & 16,000,000                     \\ \hline
% TEKGEN                                                        & 7,978,814                        & 16,090,457                     \\ \hline
% GenWiki                                                       & 1,336,766                        & 2,607,997                      \\ \hline
% \begin{tabular}[c]{@{}c@{}}LAGRANGE\\ pre-filter\end{tabular} & 37,568,527                      & 104,424,740                     \\ \hline
% \end{tabular}
% \caption{Statistics of our initial dataset and its comparison with other published datasets.}
% \label{tab:init}
% \end{table}

Once we have both $\mathcal{M'}_{\mathtt{s},\mathtt{q}}$ and $\mathcal{M''}_{\mathtt{s},\mathtt{q}}$, then we build $\mathcal{M}_{\mathtt{s},\mathtt{q}}= \mathcal{M'}_{\mathtt{s},\mathtt{q}} \cup \mathcal{M''}_{\mathtt{s},\mathtt{q}}$ to denote the set of all matched triples from $\mathcal{T}_\mathtt{q}$ to $\mathtt{s}$. Our raw dataset consists of 37 million sentences and 104 million triples. It is noteworthy to mention that 30 million triples in our initial dataset our based on second-hop neighbors of entities. Although our post-processing step filters out a number of these triples, we would like to emphasize on how going beyond first-hop neighbors can give us a dataset with higher quality, unlike other datasets that we have mentioned them in Table \ref{tab:datasets}. As we mentioned before, during the raw data collection we do not put any constraint on matching the predicates. At this stage, we just care about matching the subject and object of candidate triples with a given sentence. In the next section we describe how our post-processing step filters out triples with non-matching predicates.


==> Sections/related_work.tex <==
\section{Related Work}\label{sec:related_work}
There have been a number of previous efforts developing knowledge-graph-and-text aligned datasets, and in thiis section we discuss how our work compares to them. In general, these datasets are either high-quality but small-scale manually constructed ones such as WebNLG \citep{webnlg}), or large-scale automatically generated datasets such as TekGen \citep{tekgen}, KGPT \citep{kgpt}, GenWiki \citep{jin2020genwiki}, and WikiGraphs \citep{wikigraphs}. 

TEKGEN is a recently developed dataset that aligns Wikidata triples to the sentences in the first section of the corresponding Wikipedia articles, based on the presence of the triple object or its aliases in the sentence. 
However, its lack of predicate matching has produced graph-text pairs where sentences are aligned with the wrong triples.
KGPT, on the other hand, relies on unigram overlaps between sentences and graphs using Wikipedia hyperlinks, which can lead to missing matches for non-hyperlinked entities.
GenWiki, similar to KGPT, aligns triples and sentences based on entity set overlaps without predicate matching, but it is on a smaller scale compared to TEKGEN and KGPT.
In contrast, T-REx utilizes predicate linker and coreference resolution to match triples to sentences, but it may miss matches when the predicate is semantically entailed in a sentence but not explicitly mentioned. WikiGraphs, unlike T-REx and other previously mentioned datasets, matches entire Wikipedia articles instead of individual sentences to Freebase KG \citep{freebase}, resulting in a different scale, and it does not rely on predicate matching.

Prior works have used cyclic generation as a way of improving generative models in KG-text settings \citep{wang2023faithful,guo2020cyclegt}. In contrast, we evaluate the quality of aligned graph-text datasets by measuring the cyclic generation abilities of models trained on them.


% Human-made datasets are high-quality small-scale ones and and we have only used WebNLG \citep{} from this category for evaluation purposes. On the other hand, automatically generated datasets have significantly larger scale compared to the human-made ones. TEKGEN \citep{} is one of the most recently developed graph-text datasets. It aligns Wikidata graphs to only the root section of corresponding Wikipedia articles. More specifically, it matches a triple to a sentence in the root section if the sentence contains the object of the triple or any of its aliases. It does not perform any type of predicate matching. We will later show how this leads to non-aligned graph-text pairs. KGPT \citep{} is another recent work that is based on the unigram overlap between sentences and graphs. The major issues with KGPT are the facts that its construction does not have any predicate matching step and it is solely based on Wikipedia hyperlinks and hence misses matching a significant number of non-hyperlinked entities on Wikipedia to Wikidata graphs. Similar to the KGPT dataset, GenWiki \citep{} matches triples and sentences based on the entity set overlap. GenWiki does not perform any predicate matching and its scale is smaller than both TEKGEN and KGPT. Unlike TEKGEN and KGPT, T-REx \citep{} uses predicate linker and coreference resolution to match triples to sentences. However, the predicate linker in T-REx works based on matching the predicate or its aliases in KG to any sequence of words in a given sentence. The major problem with this approach is the fact that in numerous cases the predicate of a triple could be semantically entailed in a sentence and not explicitly mentioned and hence it will not be matched to the sentence based on T-REx construction. Finally, WikiGraphs matches Wikipedia articles instead of sentences to Freebase \citep{} KG. Since in WikiGraphs the whole article is matched instead of its individual sentences, its scale is different from previously mentioned datasets. Unlike T-REx, WikiGraphs is not constructed based on predicate matching.


%\begin{table*}[t]
%\caption{Comparing different attributes of our work LAGRANGE with other datasets. In particular and to the best of our knowledge, our work is the first to consider second-hop neighbors of the root entity during the initial matching process to increase the recall. It is also the first to apply neural predicate matching and semantic entailment to increase the precision.}
%\label{sample-table}
%\vskip 0.15in
%\begin{center}
%\begin{small}
%\begin{sc}
%\begin{tabular}{lccccccr}
%\toprule
%Property & LAGRANGE & TEKGEN & KGPT & GenWiki & WikiGraphs & T-REx & WebNLG  \\
%\midrule

%human made    & $\times$& $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\surd$ \\
%second-hop coverage    & $\surd$& $\textbf{}\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
%Non-hyperlinked annotation    & $\surd$& $\surd$ & $\times$ & $\surd$ & $\surd$ & $\surd$ & $\times$ \\
%predicate matching    & $\surd$& $\times$ & $\times$ & $\times$ & $\times$ & $\surd$ & $\surd$ \\

%semantic alignment    & $\surd$& $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\surd$ \\



%\bottomrule
%\end{tabular}
%\end{sc}
%\end{small}
%\end{center}
%\vskip -0.1in
%\label{tab:data-features}
%\end{table*}

==> limitations.tex <==
\section*{Limitations}

